HapticBots: Distributed Encountered-type Haptics for VR with Multiple Shape-changing Mobile Robots

HapticBots introduces a novel encountered-type haptic approach for Virtual Reality (VR) based on multiple tabletop-size shape-changing robots. These robots move on a tabletop and change their height and orientation to haptically render various surfaces and objects on-demand. Compared to previous encountered-type haptic approaches like shape displays or robotic arms, our proposed approach has an advantage in deployability, scalability, and generalizability -- these robots can be easily deployed due to their compact form factor. They can support multiple concurrent touch points in a large area thanks to the distributed nature of the robots. We propose and evaluate a novel set of interactions enabled by these robots which include: 1) rendering haptics for VR objects by providing just-in-time touch-points on the user's hand, 2) simulating continuous surfaces with the concurrent height and position change, and 3) enabling the user to pick up and move VR objects through graspable proxy objects. Finally, we demonstrate HapticBots with various applications, including remote collaboration, education and training, design and 3D modeling, and gaming and entertainment.

==> old.tex <==
% Section-1 INTRODUCTION
% rendering large haptic objects in VR using a synchronized movement and orientation of multiple tabletop shape-changing robots.}
% The design space and a set of haptic interaction techniques for our new concept, and its demonstration through a proof-of-concept prototype system.
% We see this as a step toward generating a fully tangible space for users working in VR adjacent to a work table.}
% \item \change{Detecting potential touch events by analyzing user's hand motion and objects placed in a VR scene, which improves the control of multiple robots to encounter the user's fingers as they reach for virtual objects. }
% \item \change{A new hardware design, inspired by shapeBots~\cite{suzuki2019shapebots} but fits the new challenging demands of a distributed haptic system, including a robust mechanical structure, precise and fast 5 DOFs  position and tilt angle and elevation control.}
% \item User evaluations that investigate the effects of \eyal{\system{} haptic illusions and compare to a simulation of prior techniques such as shape displays.}
% \item Application scenarios that demonstrate for a wide range of haptic applications enabled by \system{}.


%Mike  Contributions #5 & 6 don't appear to be true contributions compared to the normal tasks of a paper reporting user tests.



% The scalability, generalizability, portability, and simplicity of \system{} complement existing systems and can open up a new design space of highly distributed and deployable, distributed encountered-type haptic interfaces that can be easily integrated into our everyday environment. 

% \ryo{2020-09-15 Ryo: I think the current intro is a bit too long to get to the actual meat (ie., introducing HapticBots, so suggest to remove this and move to related work instead.) 

% CLAW \cite{Choi2018CLAW} managed to compress the function of grasping, texture and a one finger touch of a grounded object for a short distance, Grabity \cite{choi2017grabity} and Thor's Hammer \cite{heo2018thor} simulated grounded force interactions such as gravity. Haptic Pivot \cite{Kovacs2020HapticPivot} simulated grabbing an object thrown to or by the user. Even non-mechanically actuated systems like TORC have been envisioned to simulate grasp interactions with voice coil actuators \cite{lee2019torc}. 
% }



% ---which offer great rendering fidelity but limited range of expression---, 
% RoomShift ~\cite{suzuki2020roomshift} and PhyShare ~\cite{he2017physhare} combined multiple mobile robots to enable encountering the user hands and body in large environments where the larger distances and relatively slow motions of the users enable good prediction of touch events.
%These encountered-type haptic devices include using shape-changing displays to render various shapes (e.g., shapeShift~\cite{siu2018shapeshift}), a robotic arm to simulate graspable objects (Snake Charmer~\cite{araujo2016snake}), and combining mobile robots and haptic props to provide large-scale haptic interaction (RoomShift~\cite{suzuki2020roomshift}, PhyShare~\cite{he2017physhare}).

%In particular, {\it encountered-type haptics} has been introduced as an emerging new approach to providing haptic sensations by {\it reconfiguring %physical environments}.
%The encountered-type haptics promise more immersive haptic experiences, simulating larger-scale surrounding environments, which is often difficult %to emulate with only common handheld or wearable haptic devices

%For example, these systems often require large and mechanically complex systems, thus it is not easily deployed on demand. Also, shape displays promise to render various shapes, but its interaction area tends to be small and fixed because of the expensive and complex form factor. Finally, using a single robotic arm or mobile robot tends to lack the generalizability to support various applications. 

%While past approaches pose interesting directions, their limitations and complexity often limit the generality of their use and their availability outside research labs. Complex, expensive and heavy mechanical systems that are hard to move and may even pose a danger are not easily deployed in everyday spaces. Many of the systems are limited in the area they may cover by their reach or sensing and are hard to be mobilized on demand,  reducing their usability to researchers, developers and users. 

%by leveraging tabletop-scale swarm robots that can dynamically simulate various objects and surfaces in VR.
%To this end, we introduce \system{}, tabletop-scale shape-changing swarm robots, that enables a distributed encountered-type haptic sensations.

%

%Inspired by recent shape-changing swarm robots~ (e.g., ShapeBots~\cite{suzuki2019shapebots}), we developed a novel shape-changing swarm robots that %are compact (e.g., 5 $\times$ 5 cm in size, 8 cm in height), highly extensible (e.g, from 8 cm to 30 cm), stable with strong force (e.g., withstand %500 g), fast travel (e.g., 3 cm/sec), and tiltable to various angles (e.g., from -50} to 50} degree).
% and relatively inexpensive (e.g., 70 USD).


%Due to these advantages, our proposed approach of using shape-changing swarm robots for encountered-type haptics enables the numerous advantages in %deployability, scalability, and generalizability, compared to previous shape displays or robotic arms approaches.
%This approach would provide a complement of existing systems and can open up a new design space that is highly distributed and deployable %encountered-type haptic interfaces that can be easily integrated into our everyday environments.
%In addition, our robots can be easily customizable with passive haptic props, which can be useful for many different custom applications.

%\eyal{{\bf Eyal: Let's move the detailed description (cm, weight, size, range) to the implementation section:} 
%\footnotesize
%\system{} consists of up to seven tabletop-scale shape-changing robots.
%These robots move on a tabletop and change their height to simulate various virtual objects and surfaces by providing on-demand haptic sensations in %VR.
%Inspired by recent shape-changing swarm robots~ (e.g., ShapeBots~\cite{suzuki2019shapebots}), we developed a novel shape-changing swarm robots that %are compact (e.g., 5 $\times$ 5 cm in size, 8 cm in height), highly extensible (e.g, from 8 cm to 30 cm), stable with strong force (e.g., withstand 500 g), fast travel (e.g., 3 cm/sec), and tiltable to various angles (e.g., from -50 to 50 degree).
% and relatively inexpensive (e.g., 70 USD).
%By combining with the commercially-available off-the-shelf robots, these robots can be used to provide various haptic sensations for virtual and %augmented reality environments.}


%Due to these advantages, our proposed approach of using shape-changing swarm robots for encountered-type haptics enables the numerous advantages in %deployability, scalability, and generalizability, compared to previous shape displays or robotic arms approaches.
%$This approach would provide a complement of existing systems and can open up a new design space that is highly distributed and deployable %encountered-type haptic interfaces that can be easily integrated into our everyday environments.
%In addition, our robots can be easily customizable with passive haptic props, which can be useful for many different custom applications.


% such as virtual object manipulation, 3D modeling, remote collaboration, entertainment, education, and remote operation. 
% Currently, however, most virtual objects lack haptic sensations. Users cannot physically interact, touch, or grab them, which significantly limits the sense of full immersion of the virtual world. Thus, there is a clear need to provide better haptic sensations in VR.
% Various haptic devices have been explored to address this problem. For example, hand-held controllers and other wearable haptic devices~\cite{choi2016wolverine, choi2018claw, heo2018thor, Kovacs2020HapticPivot, lee2019torc} were developed to generate compact and light force haptic sensations on the user's hands or fingers with impressive rendering capabilities. 
% However, portable hand-grounded devices are inherently limited in their ability to render a sensation of earth grounded objects.


% robot and their synchronization to simulate large geometries and objects, much larger than the size of the robots combined (Figure \ref{fig:teaser} d & a).
% thus giving the illusion of rendering a rigid surface which is larger than the robots. 

% \eyal{In contrast to the existing mobile robotic haptic devices (e.g., PhyShare~\cite{he2017physhare}), or MIT's Hermits \cite{nakagaki2020hermits}, that used each robot of a swarm to render one single object out of predefined geometries, \system{} 
% leverage the shape-changing capability of 


% These features enable \system{} to support many different applications, including remote collaboration, education and training, design and 3D modeling, and game and entertainment.
% We see such a solution a possible architecture for general haptic solution for VR users that work sitting at a desk.
% \eyal{
% We build a system that is simple and affordable yet general for many applications. 
% Following the design of  who used table-top consumer robots to generates 2D visual displays, we used 
%  }

% HapticBots travel quickly to reach the user's hands in time for the expected touch. This makes HapticBots a safer alternative to robotic arm options like Snake Charmer \cite{araujo2016snake}. 
 %\mar{mike comment: Example applications?}
% Replacement of the robot's planar touch surfaces with other passive proxies can enable  customization of the haptic touch sensation for


% , in which haptic sensations are provided through {\it actuated physical environments}~\cite{mcneely1993robotic}.

% Encountered-type haptics have many benefits, including  a true sensation of large-scale surrounding objects and surfaces~\cite{cheng2015turkdeck, suzuki2020roomshift}.


% passive haptic objects of fixed geometry~\cite{hettiarachchi2016annexing} 

% , which use a matrix of actuators to render a 2.5D shape, 
% while using a relatively large number of actuators (between tens to hundreds), 

% scalability problem: when increasing a number of robotic arms, it becomes more difficult to control without collisions


% large and heavy systems like shape displays~\cite{siu2018shapeshift, iwata2001project,nakagaki2019inforce} or robotic arms~\cite{vonach2017vrrobot}.


% For example, in contrast to non-transformable mobile robots which can only render a single predefined object~\cite{he2017physhare, gonzalez2020reach}, our approach can simulate various haptic geometries like continuous surfaces with concurrent height and position change.
% , while maintaining compactness of the system and a deployable form-factor
% By leveraging both transformation and locomotion capability, they can


%\eyal{ The area is defined by the area of a printed pattern paper mat used by the robots for location tracking. It may be extended using a larger printed pattern.} 
% Thus, we made the following technical contributions beyond the prior works:
% For example, \system{} can resist human-scale forces with the capability of withstanding a 13.5N downward force when extended at 25cm and 21.8N when only 12cm high.
% We further build the sensing and control software by integrating with Oculus Quest's hand tracking.
% {\it 3) Tilt surface support:} The closed-loop control also allows the precise tilt control to render various surfaces with varying normal directions from -60 to 60 degree.
% {\it 4) Deployable tracking system:} \system{} reduces the requirement of dedicated tracking system (e.g., transparent desk and mounted camera in~\cite{suzuki2019shapebots}) by leveraging easily deployable and expandable tracking mechanism based on a paper mat.
% {\it 4) VR applications:} 
% Finally, and most importantly, our work, to best of our knowledge, is the first demonstration of using tabletop-size shape-changing robots for haptic interactions in VR.

% and easily changed of geometry using small battery-operated motors, span of a large height dynamic range and resist human forces.
% The design and implementation of \system{}, including a number of technical improvements beyond a similar system\cite{suzuki2019shapebots}, such as a highly robust and extendable mechanical structure, 
% which is suitable for VR haptics and a software platform that can synchronize VR and physical environments. 
% \eyal{While the initial design was inspired by ShapeBots , } 

% Based on our user study feedback, we have developed various application scenarios.





% Section-2 RELATED WORK



% Therefore, a novel software and hardware system is needed to appropriately support VR haptic experiences.
% to the user visually and  haptic rendering sporadically wherever the user reaches her hands to touch the object. 
% , which we believe opens up a new possibility for encountered-type haptic interactions.

% In summary, our work, to best of knowledge, is the first exploration of employing tabletop shape-changing multi-robots for VR haptics, which opens up a new possibility for robotic haptic devices.
% We contribute to a novel set of interactions enabled by the combination of the robot's mobility, shape-changing capability, and coordinated behaviors.




% By leveraging modular extendable actuators, similar to G-Raff~\cite{kim2015g} and Kinereels~\cite{takei2011kinereels}, 

% Most closest to our work, introduce the concept of shape-changing swarm robots to expand the tangible interaction with swarm robots. 

%and this paper contributes to expanding the application of these robots for encountered-type haptics in VR, .

% A swarm of robots generally can approach the users’ different body parts and when close to the user they can act as haptic display patterns that vary in spatial, temporal, and force coordination \cite{kim2019swarmhaptics,kim2017ubiswarm}. 


% These interfaces can be promissing to provide dynamic haptic sensation for VR.
% There is HapticSwarm, but not for VR.
% ShapeBots is the closest, but we need to reconsider the mechanical design. 
% G-Raff.
% Our work is the  first at exploration the use of  tabletop-scale swarm robots for encountered-type haptics for VR.

% \subsection{Human-Robot Interaction with Swarm Robots}
% Outside of the context in haptics for VR, our work is also inspired by an emerging area of human-robot interaction, particularly with swarm robots~\cite{le2016zooids, kim2017ubiswarm}.
% Some existing works explore the use of these small tabletop robots for everyday haptic feedback~\cite{guinness2018haptic,kim2019swarmhaptics, suzuki2017fluxmarker} or constructing haptic proxy objects for VR~\cite{zhao2017robotic}.
% We extend these works by exploring the large-scale haptic feedback, inspired by the concept of shape-changing swarm robots~\cite{suzuki2019shapebots}.
% In the context of human-robot interaction, some works integrate wheeled robots with furniture for spatial reconfiguration.
% For example, Mechanical Ottoman~\cite{sirkin2015mechanical} adds a wheeled robot to existing furniture to make it autonomously mobile. Similarly, shape-shifting wall displays move to adapt to the content projected on the wall~\cite{takashima2016study}.
% We extend prior work on robotic furniture by investigating its use for haptics in VR and proposing the required technologies and interaction techniques unique to VR applications.



% However, most robotic haptics work at the scale of the human hand and achieving a larger-scale robotic haptic experience presents significant design and technical challenges including flexibility, scalability, robustness, and deployability. This paper contributes to the exploration of large-scale robotic haptic interfaces by deploying a swarm of shape-changing robots to provide dynamic large-scale haptic sensations. 


% This paper extends this line of work in two ways: 
% First, in contrast to a single robot, we deploy a swarm of coordinated robots, which provides faster spatial transformation for haptic interfaces as the workload can be divided.
% Second, instead of emulating an object with the robot itself we propose moving furniture with robots, which can provide a more robust structure which the user can interact (e.g., sit on, place on, step in, and lean against),
% Once an object is relocated, it serves as static and robust furniture, so it can support a range of interactions while maintaining the dynamics and fluidity of the environment.

% This paper extends these lines of work in two ways: 
% to provide large-scale haptic feedback that users can interact with their whole body.}
% combining the passive haptic proxies with object actuation.
% In this way, we can provide a dynamic haptic environment that is 
% which can provide a more robust structure which the user can interact with the whole body.}


%The robots can generate significant Resistance to the user's pressure but light and enable manipulation of virtual object by pushing or grabbing and moving the robots along the desk.

%but in contrast to existing approaches, we aim to emulate the whole environment of the virtual space. 


%The other approach of active haptic feedback is {\it encountered-type haptics}, in which haptic devices dynamically deliver physical props when the user makes contact with a virtual object.
%Unlike the wearable approach, the encountered-type approach augments the environment, instead of the user's body.

%We achieve this by combining passive objects with robotic actuation. 
%Instead of emulating building elements with the robot itself, we propose actuating furniture with robots, which allows more robust and %larger-scale haptic feedback for VR.

% \subsubsection{Large-scale Encountered-type Haptic Feedback}
% Prior work on exploring large-scale haptic feedback has focused on reconfiguring the physical environment around the user.
% %HapticTurk~\cite{cheng2014haptic} used human helpers that lift and tilt a player to produce a physical sensation in a video game.
% TurkDeck~\cite{cheng2015turkdeck} leverages human volunteers to help to reconstruct the space for realistic haptic feedback. However while 
% %The human actuation approach~\cite{cheng2018iturk, cheng2014haptic,cheng2017mutual,cheng2015turkdeck} is 
% intriguing for prototyping or simulating the large-scale haptic feedback, requiring a group of human helpers is limited in availability and scalability. % as it always requires a group of human helpers to achieve the experience.
% Room-scale systems such as TilePoP~\cite{teng2019tilepop} and LiftTiles~\cite{suzuki2020lifttiles} investigate the use of inflatable actuators to dynamically change the environment to provide a haptic proxy.
% Although inflatables are safe and low-cost, they are also slow: the speed of transformation and degrees of freedom are key limitations to providing real-time dynamic haptic sensations.

% To overcome these limitations, \system{} explores a swarm robotic approach to reconfigure the environment. This benefits from a faster spatial transformation which is important for the real-time synchronization between virtual and physical environments.


% However, portable hand-grounded devices are inherently limited in their ability to render a sensation of earth grounded objects.


% In recent years researchers have explored active haptic feedback in the context of wearable or hand-held devices. This enables the users to roam around and experience larger virtual scenes. 

% Other devices rendered fingertip sheering \cite{whitmire2018haptic}, vibro-tactile texture \cite{Choi2018CLAW} and even simulation of external and grounded forces such as gravity\cite{choi2017grabity} and Inertia ~\cite{heo2018thor, sasaki2018leviopole, shigeyama2019transcalibur}.




%beyond the human hands~\cite{lindeman2006wearable}. wearable haptic suits~\cite{nagai2015wearable, delazio2018force}, actuated %shoes~\cite{schmidt2015level} have been proposed to provide haptic feedback to the user's body.
%still limited to emulate a whole environment, which is the focus of our work.



% For example, CLAW~\cite{choi2018claw} supports the function of grasping, texture, and a one-finger touch of a grounded object for a short distance. 
% Grabity~\cite{choi2017grabity} and Thor's Hammer~\cite{heo2018thor} simulated grounded force interactions such as gravity. Haptic Pivot \cite{Kovacs2020HapticPivot} simulated grabbing an object thrown to or by the user. Even non-mechanically actuated systems like TORC have been envisioned to simulate grasp interactions with voice coil actuator vibrotactile illusion of compliance~\cite{lee2019torc}.

% Robotic encountered-type haptics is first introduced by McNeely. 
% His concept of Robotic Graphics envisions the simulation of haptic sensations by {\it physically reconfiguring the environment}. 


% can split the interaction space, and reduce the distance that each robot has to move to encounter users' hands.}
% CirculaFloor~\cite{iwata1999walking} used multiple movable robots to simulate dynamic terrain on which the user walks. Recently, drones and wheeled robots have  also been proposed as a way to move proxy objects for encountered-type haptic experiences.



% retargeting to expand the spatio-temporal reachable space of mobile robots.
% In contrast to these existing mobile robotic haptic devices, \system{} leverage the coordinated behavior of multiple robots and their shape-changing capability to simulate both \eyal{continuous virtual surfaces as well as seperated graspable objects, which allows for greater flexibility for general-purpose applications.}\\
% \eyal{{\bf Eyal: This point is not clear: Doesn't CirculaFloor render a continuous surface? Does other not render graspable objects? In any case, I would ALWAYS put the more advanced, continuous surface capability first.}} \\

% ~\cite{le2016zooids}.
% Swarm user interfaces are a class of computer interfaces that leverage many collective mobile robots for tangible interactions~\cite{le2016zooids}.
% There have been a number of examples in this area of research



% In recent years, various haptic devices have been explored to enhance the immersion of VR. We first review different approaches of haptic interfaces.


% They were developed to generate compact and lightweight force haptic sensations on the user's hands or fingers.
% Prior systems generate haptic feedback through small finger-tip or palm size shape displays, rendering forces between the fingers, and wrist-based actuated objects to add forces on the palm. 

% , simulating the resistance to the penetration of the fingertip into the virtual object. 

% Other approaches such as electrical control of muscles~\cite{lopes2015impacto} might also have future potential for encountered haptic sensations, the research has to yet reach an acceptable fidelity for the public, among other problems.
% This approach enables a simple, reliable, and inexpensive way to provide haptics the VR user may pick them up or touch.
% , without the requirement of a complex mechanical actuation.
% Such physical props are often not in constant contact with the user's hands. 
% Occasionally, the user may pick them up or touch them. Such interaction is called {\it encountered-type haptics}. 
% Various works have been explored for this type of haptic feedback. 

% Also, while using a relatively large number of actuators (between tens to hundreds), the resolution of the display are still limited, making it difficult to render a smooth and continuous surface. 
% However, they only render a single predefined object due to the lack of transformation capability.
% On the other hand, \system{} only renders the geometry at the points of contact between the virtual objects and the user's hands. 
% \system{} can render virtual surfaces that span along a larger interaction space, as well as dynamically moving objects, using a limited number of robots.
% Overall, \system{} is categorized as robotic encountered-type haptics, mixing advantages from past approaches: it uses a small swarm of tabletop-size robots to encounter transforming a desk into a continuous shape display on-demand. 






% Section-3 CONCEPT


% \begin{figure}[h!]
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \includegraphics[height=0.85\textwidth]{draft-figures/House_Multi_Bots.png}
% }
% \caption{Coordinated behaviors with multiple robots. \eyal{While each robot can only render a planar patch of the objects around a finger touch point, multiple synchronized robots can generate more complex geometry (left). The robots may use also their base geometry to approximate geometry close to the desk (right).
% Multiple touch points can enable the user to move, rotate or scale virtual objects.}}
% ~\label{fig:coordinated-multiple-robots}
% \end{figure}



% many of rendered virtual objects 
% the entire geometry exists in the physical world. 

% \eyal{Another possible strategy is aligning robots adjacent to each other to form a larger touchable surface. As the user movers their hand along the surface, it is possible to use robots that have already been touched but no longer in hand-contact,  to move to a new location to maintain an illusion of a large  object.}

% These proposed interaction techniques promise various application scenarios enabled by \system{}.
% \eyal{Currently, picked robots have a fixed rectangular shape, but following  \cite{nakagaki2020hermits}, we can see opportunity to change the robots tangible geometry by picking up special robot covers that can be positioned in pre-known locations.
% } 
%In contrast to shape displays, each compact robot is not bounded to the surface and can be picked up by or returned to the display surface by the user.


% \subsubsection{Customizable Haptic Props}
% Each \system{} robot is composed of three main functionalities (Figure~\ref{fig:concept} bottom right). The base cube-like robot moves the robot along the desk or the display surface. The elevation mechanism controls the height and orientation of a top planar surface, and the top surface is the part that approximates the virtual geometry.
%It is also easy to customize and augment existing robots.
% \eyal{The Hermits system ~\cite{nakagaki2020hermits} introduced the ability for robots to reconfigure their mechanical shell. In VR, the dominance of the visual sense enables more variations between the proxy geometry and the visuals, yet we could use a similar idea and attach various haptic props on top of the robot's top surface. This way it is possible the vary the geometries, the surface textures, and even materials that the user can feels when touching the robots. (Figure~\ref{fig:concept} bottom right). It may also open options such as adding physical widgets such as buttons.}
%mike There's a lot of "This could..." or Our system is capable of ..." where we haven't actually done it. We have to be careful of claiming too much that hasn't been done yet. We should probably move this and other conjectures to Future Work. 

%For example, attaching surfaces of different texture, different haptic prop shapes and tactile mechanism (e.g., buttons with 3D printed parts and spring).
%for each robot, these robots can emulate various texture, similar to a reconfigurable controller of NormalTouch and TextureTouch.
%By leveraging multiple robots that have a different texture, we can emulate a different texture surface by locating them appropriately.
%Not only for textures, but we can also support different haptic prop shapes (e.g., attached sphere for moving sun and earth) and tactile mechanism %(e.g., buttons with 3D printed parts and spring).
% It is also possible to combine with other materials to emulate various haptic sensations (e.g., attaching a string for fishing).


% \begin{figure}[h!]
% \centering
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{draft-figures/table.jpg}
% }
% \caption{table}
% ~\label{}
% \end{figure}


%This section introduces a novel concept of {\it distributed} encountered-type haptics.
% \subsection{Seven Unique Features in Our Approach}



%Encountered-type haptics enabled by mobile robots can cover a large and flexible interaction area.
%For example, these robots can simulate haptic proxy objects or surfaces regardless of the limitation of the size of the robot itself.
%This is a unique contrast to shape display approaches such as Feelex~\cite{iwata2001project} and inForce~\cite{nakagaki2019inforce}, which are usually %limited with fixed and immobile interaction space.
%While some of the shape display explores the mobility (e.g., shapeShift~\cite{siu2018shapeshift}), by leveraging the multiple robots, these robots can %cover a larger-size area that can fully leverage two-handed interactions. 
%Also, interaction areas do not need to be a square shape. 
%As these robots can move to an arbitrary surface, interaction space is flexibly defined.
%By mounting onto a tilted or vertical surface, it could be also possible to provide similar encountered-type haptics for both horizontal and vertical %surfaces. This enables a richer experience that requires mid-air interactions (e.g., Sparse Haptics). 

%\begin{figure}[h!]
%\centering
%\resizebox{1\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{draft-figures/terrain.jpg}
%}
%\caption{}
%~\label{}
%\end{figure}


% require a large, heavy, and mechanically complex systems, which makes it difficult to bring and deploy.
% Thus, these devices often only work in a specific installed place, such as a laboratory.
%One of the inherent disadvantages of encountered-type haptics---compared to handheld or wearable approaches---has been its portability and deployability of the system.
%Our approach can mitigate this problem as each robot is compact and small enough to deploy everywhere.

%Since our robot's form factor is also compact, the overall system is easily deployable.



%user and interact with them.
%The compact form factor of each robot also contributes to this feature.
%Compared to the previous mobile robotic haptic devices, the small-size of robots allows the user to grasp with one hand.
%This feature is particularly interesting when the user needs to freely pick up virtual objects.
%For example, when picking up a robot and use the robot's surface like a touchpad of a menu, then it is much easier to interact with these virtual menus. 


% renders a single sample of the virtual surface, at arbitrary position and orientation over the display area. Furthermore, the robots 


%Another unique advantage of 
%For example, the shape display does not fully support this feature.
%Since pins are attached to the base plate, each pin can support vertical movements (i.e., moving up and down), the lateral position of each pin cannot move.

%By leveraging this capability, our approach enables a couple of unique interactions. 
%For example, these robots can support interactions that require lateral movements, such as a slider and a wheel handle.
%By combining the height-changing capability, our approach can support much richer haptic interactions.
%For example, by continuously moving and changing the height of robots, \system{} can support a continuous curvature of the virtual surface.
%This is a particularly unique and previously unexplored haptic modality, as most of the existing systems leverage a number of pins to render a shape. 

%This approach, although relatively high resolution, cannot simulate the continuous surface as there are inherently gaps or seams between each pin. 
%Thus, this introduces an interesting research question in which how the user perceives the continuous curvature enabled by \system{} and how the %experience can be different from the rendered shape with discrete elements. 




% \subsection{Overview}

% \begin{figure}[h!]
% \centering
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=\textwidth]{draft-figures/top-1.jpg}
% % \includegraphics[height=\textwidth]{draft-figures/top-2.jpg}
% \includegraphics[height=\textwidth]{draft-figures/top-3.jpg}
% }
% \caption{\system{} can render surfaces with multiple coordinated robots, or through a single robot that follows the user's hand in anticipation of a touch.}
% \Description{}
% \label{fig:overview}
% \end{figure}


% \system{} is a swarm of self-transformable robots that are specifically designed to provide encountered-type haptics for VR.
% \system{} consists of custom designed, extendable, reel-based linear actuator and base mobile robots.
% By dynamically changing their height, position, and orientation, these tabletop-scale robots can haptically render various surfaces of virtual objects on-demand. 
% We call this new encountered-type haptic approach enabled by shape-changing swarm robots as {\it distributed} encountered-type haptics in which the robotic encountered-type haptic devices are distributed in the space to enable a large and flexible interaction space.
% This section first introduces this new class of systems and describes the unique features and a set of interaction techniques, enabled by \system{}. %Then, we describe software and hardware design and implementation of \system{} system.
% \eyal{Eyal: These are only 3. You can refer to the to plane, as a passive haptic element that can be ranging from a plane, to other shapes, to interactive buttons.}



% Compared to previous encountered-type haptic approaches, our proposed approach has advantages of deployability, scalability, and generalizability.

% \subsection{Distributed Encountered-type Haptics}
% We believe HapticBots is the first system of VR haptic interaction with tabletop-size shape-changing swarm robots, which enables a set of previously unexplored haptic interactions.
% We call this new approach {\it distributed} encountered-type haptics, a new class of haptic interaction enabled by distributed and synchronized mobile robots.
% To better understand this new class of the haptic systems, we first describe the potentials and unique advantages of distributed encountered-type haptics.



% Compared to prior tabletop-scale encountered-type haptics (e.g., haptic shape displays or robotic arms), our approach has the following unique capabilities (Figure \ref{fig:concept}):
% \begin{enumerate}
% \item Large and flexible interaction area.
% \item Accurate 3D positions and 2D surface orientation rendering.
% \item Coordinated behavior to render multiple concurrent touch points, generating the illusion of a large physical object.
% \item Each robot can simulate a graspable object
% \item Portable and deployable form factor
% % \item Customizable touch surface with haptic props 
% \end{enumerate}



% The robots can easily reach over a desk or floor, or moving between obstacles and planar areas of arbitrary shapes.
% In this paper we only employ horizontal surfaces, yet by using tilted or vertical surfaces and attaching the robots to the surface, it is possible to provide a similar angled or vertical interaction space. 
% For example, the previous approaches like shape displays~\cite{follmer2013inform} cover a fixed area, and are usually used in one location. While shapeShift~\cite{siu2018shapeshift} explored moving a shape display, its weight limits the speed it may move close to a user's hand. In a similar way, large robots arms may reach large areas but are limited, mainly due to safety issues.

% Due to their large size and weight, many existing encountered-type haptics, such as shape displays or robotic arms, are often deployed to static locations.

%Lateral and Continuous Movement}


% be positioned and rotated freely to render the correct position and orientation of the virtual surface, wherever the user's fingers encounter it, giving an illusion of the existence of a large object in the space.

% While not rendering the friction force with the surface as the finger 'travels' along the virtual object, the rendering of the normal force to the surface that prevents the finger from penetrating the object generates a strong illusion of a continuous virtual surface.
% Mike - Isn't this is pushing it a bit as it probably takes a lot more work to enable our bots to correctly follow a finger(s) movement when in contact with a robot....or have we shown we can indeed do this with accurate coordination?}


% Similar to prior haptic interactions with multiple robots (e.g., Circular Floor~\cite{iwata1999walking}, RoomShift~\cite{suzuki2020roomshift}),
% The coordination of multiple robots extends their rendering capabilities and expressiveness.


%By changing their individual height accordingly, the robots can also mimic a low-resolution shape display, in which each tile of the surface dynamically moves and actuates.This enables the system to simulate various surfaces and objects, such as a roof of a house with two tilted surfaces.


% Section-4 System

%do the same process at offset point (i.e., $(x_1, y_1)$ and $(x_2, y_2)$, where $x_1, x_2 = x \pm \delta$ and $y_1, y_2 = x \pm \delta$, and use the %height of each point i.e., $height_{(x_1, y_1)}$ and $height_{(x_2, y_2)}$ to specify the height of each actuator.
%The reason why we ray cast from the top instead of the bottom is the ray cast sometimes does not work from the inside of the object.
%While this approach cannot detect the internal surface, this approach can detect the appropriate top touchpoint of the convex surface (e.g., a top %surface of a cube with a hole). 


% \subsubsection{Different Target Assignment for Different Interaction Modes}
% Different target assignments for robots can support different modes of interactions such as static haptic proxy, inter-material interactions, and continuous surfaces. 
% For example, 
% %instead of continuously assigning the target position to the finger position, 
% we can assign the target position to each of virtual objects (e.g., virtual houses, buildings, and cars on a map example), using the robots as haptic proxy objects of either static (such as buildings) or dynamic (e.g., moving cars).
% %By leveraging the combination of hand tracking and dynamic target assignment, the smaller number of robots can simulate more virtual haptic proxy. 
% Based on the user's hand position, the system prioritizes the robots for objects that are close to the current hand position, enabling the robots to haptically simulate a larger number of objects. %\eyal{Eyal: How many can you simulate with a given 'k' robots. I know it is hard to estimate, but if you have 1 robot - how far can a hand move and still have the robot manage to get to the next touch point? }
% %so that the robots can position to the virtual objects close the hand, while the virtual objects that are far from the hand leave without haptic proxy.

% \\Therefore, we do not require any environmental tracking system. 
%Rather, it works on a portable marker-printed mat or paper that can be easily deployed in any place, which was one of our design requirements.

% While the hardware itself is designed to work only with an accompanied gaming console and cartridge, w

% \begin{figure}[h!]
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{draft-figures/vr-concave-horizontal-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{draft-figures/vr-concave-horizontal-2.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{draft-figures/vr-concave-horizontal-3.jpg}
% }
% \caption{A single robot simulates a concave shape.}
% ~\label{}
% \end{figure}


%\resizebox{0.49\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{draft-figures/vr-sphere-horizontal-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{draft-figures/vr-sphere-horizontal-2.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{draft-figures/vr-sphere-horizontal-3.jpg}
%}
%\resizebox{0.49\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{draft-figures/vr-concave-horizontal-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{draft-figures/vr-concave-horizontal-2.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{draft-figures/vr-concave-horizontal-3.jpg}
%}
%\includegraphics[height=1\textwidth]{draft-figures/Sphere_conacave.jpg}

% \subsubsection{Interaction Capability}
% %We can use the same mechanism to track user input. 
% The system supports four different types of user interaction that our system supports: place, move, orient, and pick-up. 
% % mike  maybe choose different terms. place, move, orient, and pick-up aren't necessarily interactivity terms so much as degrees of freedom. \eyal{{\bf Eyal: } Might worth a bit longer description: Is place a manual placement by the user or by the system? If the later, what is the difference than 'move'?}
% When the user grabs a virtual object, the system stops controlling the robot and lets the user move it, so that the user can  place the virtual object at a new location.
% By leveraging the robot's localization capability, the system can also detect where the user moves or places the robot, which can be useful for remote collaboration settings (e.g., when the user moves one robot, then the virtual objects and robots in the remote environment can also synchronize their positions simultaneously.)


% A single user can also manipulate multiple robots with two hands (e.g., using two robots to zoom in/out on a map application).
% This user interaction capability is also useful for remote collaboration. 
% For example, when the user moves one robot, then the virtual objects and robots in the remote environment can also synchronize their positions simultaneously.
% While the robot does not have a force sensing, the user can use the Oculus controller as a force sensitive input.
% %\eyal{Eyal: I would put it in a positive form: The robots are designed for direct touch interaction, yet it is also possible to use them along with other devices such as the Oculus controllers. Tracking the controllers it is possible to detect a collision with the robots, and simulate interaction such as a minecraft hammer that cause the robots, representing the ground, to change their height.}  \\
% %\eyal{Eyal: I'm not sure how you get force or pressure from the rear grip. - maybe we should just refer to touch events.}
% For example, by using a rear grip of the Oculus controller to touch the surface, the system can measure how much the user pushes the surface.
% With this capability, the system can also support various input modalities, such as sculpting in 3D modeling or digging blocks in Minecraft application. 

 

% \begin{enumerate}
% \item Load-bearing capability of the linear actuator 
% \item Maximum force of vertical extension until the actuators stall
% \item Force exerted by the robot when horizontally pushing external objects
% \item Speed of vertical extension of the linear actuators
% \item Speed of horizontal movements of the robot
% \item Moving to target times of the robots
% \item Accuracy of the vertical extension of the linear actuator
% \item Accuracy of the tilting of the linear actuators
% \item Accuracy of the robot control system in position and orientation
% \item Latency of a control loop with the Computer
% \end{enumerate}

% Figure~\todo{X} shows the graph plot of the distance and average reach time.
% The graph indicates that the robot can reach to the position within \todo{0.8} seconds on average and at least \todo{1.4} seconds at the furthest distance.

% \subsection{Design Goals and Requirements}
% When we explored mobile robotic-based encountered-type haptics, we immediately identified that only mobility may not be enough to support a variety of interactions. For example, a simple mobile robot can provide haptic sensations on a ground surface where this form factor significantly limits the haptics above the tabletop surface. 
% \eyal{Fixed shape robot that can only move on a 2D surface is very limited in its expresibility. To enable generality, we designed a shape changing robot.} Therefore, we have decided to explore the shape-changing capability of each robot to expand the range of interactions and possible applications.
% \eyal{As our robots mobility is limited to lateral movement (i.e. X-Y directions), the shape chaning sub system of the robot aims at enabling vertical geometry such as changing heights and surface normals.} 
% %One promising shape-changing modality is the height changes, as the mobility of robots can cover lateral movement (i.e., X-Y direction), thus by supporting the missing vertical movement (i.e., Z direction) with the additional height change, 
% %we hypothesized that it can expand the possibilities.
% %Also, as we mentioned in the previous section, we aim to support various features that are missing in the current encountered-type haptic devices. 

% %Therefore, 
% Our design goals are 
% \begin{enumerate}
% \item Compact and graspable form factor  \mike  [Is "graspable" a main goal?]
% \item Easily deployable tracking system
% \item Mechanical stability for haptic interactions
% \item Fast XY movement and Z-extension for real-time interactions
% \item Sufficient force and stiffness to enable human touch
% \end{enumerate}
% \eyal{Eyal: This is a repetition of past section}



% \begin{figure}[h!]
% \centering
% \includegraphics[width=1\columnwidth]{draft-figures/hapticbots.jpg}
% \caption{hapticbots}
% ~\label{fig:system-overview}
% \end{figure}

% \begin{figure}[h!]
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{draft-figures/angle-1-crop.jpg}
% \includegraphics[height=1\textwidth]{draft-figures/angle-2-crop.jpg}
% \includegraphics[height=1\textwidth]{draft-figures/angle-3-crop.jpg}
% }
% \caption{The cap can tilt up to 60 degrees.}
% ~\label{fig:system-tilt}
% \end{figure}



% \begin{figure}[h!]
% \centering
% \resizebox{0.7\columnwidth}{!}{
% \includegraphics[width=1\textwidth]{draft-figures/load-bearing-1.jpg}
% \includegraphics[width=1\textwidth]{draft-figures/load-bearing-2.jpg}
% }
% \caption{The actuator maximum holding load is 1379 g at the extended state (25 cm height).}
% ~\label{fig:system-load}
% \end{figure}



% \eyal{, which was sufficient for all our experiments and we did not need more robots.} 
% mike  Please explain how BTLE has to do with # of robots required.
% \eyal{{\bf Eyal}: This is not an inherent limitation of the proposed paper. Should we say that by replacing the communication channel it is possible to increase the number of bots?}% mike  pls, more detail. Is this PC and Robots in their control loop?



% Section-5 USER STUDY 


% With this task we aim at studying the performance of \system{} in two areas: 1) ability to render tilted surfaces and provide that information to the users; 2) generate a continuous touch sensation when participants explore continuous tilted surfaces. 

% Continuous touch fidelity is generally hard to achieve with regular pin-based shape displays where users experience aliasing as they move over non-horizontal surfaces. Some work has attempted to reduce aliasing by using redirected techniques \cite{abtahi2018visuo}.
% However, the continuous touch experience is often disrupted on shape displays. 
%mike   you describe the tilt range is only -60 to 60 degrees. 








% Section-6 APPLICATIONS


%Mike   I believe a missed topic is for an accessibility display for the visually impaired person (VIP). I think this could be an absolutely great tool for the VIP to read a 3D map, discover height problems for wheelchair users, playing (VR) games with their sighted counterparts, planning furniture placement for best use, live performances, etc.



%\subsubsection{3D Modeling}

%\subsubsection{Painting}


% To better understand the design space of this novel encountered-type haptic approach, we propose a set of interaction techniques enabled by shape-changing swarm robots.
% For example, these robots can simulate a continuous surface by both moving and changing their height which can physically synchronize between the user's finger position and the current height of a virtual surface. They can be interacted with one or two hands.
% Also, these robots can simulate various surfaces and objects by leveraging multiple robots in coordination, such as a roof of a house with multiple connected tilted surfaces or buttons or sliders with independently moving robots, or using the robot sides to represent vertical walls of the house which the user may push to move the house around. Such proposed interaction techniques promise various application scenarios enabled by \system{}. 


%\begin{figure*}
%\centering
%\resizebox{1\textwidth}{!}{
%\includegraphics[height=\textwidth]{application-figures/house-7.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/minecraft-2.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/body-2.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/mountain-4.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/cockpit-3.jpg}
%\includegraphics[height=\textwidth]{application-figures/chess-3.jpg}
%}
%\resizebox{1\textwidth}{!}{
%\includegraphics[height=\textwidth]{application-figures/house-7-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/minecraft-2-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/body-2-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/mountain-4-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=\textwidth]{application-figures/cockpit-3-1.jpg}
% \includegraphics[height=\textwidth]{application-figures/chess-3-1.jpg}
%}


% \begin{figure*}[h!]
% \centering
% \includegraphics[width=1\textwidth]{draft-figures/application-scenarios.jpg}
% \caption{Application scenarios.}
% ~\label{fig:application-sketches}
% \end{figure*}



%\begin{figure}[h!]
%\centering
%\resizebox{1\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{application-figures/chess-2.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/chess-3.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/chess-4.jpg}
%}
%\resizebox{1\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{application-figures/chess-1-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/chess-3-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/chess-4-1.jpg}
%}


% \begin{figure}[h!]
% \centering
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{application-figures/cockpit-6.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/cockpit-3.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/cockpit-4.jpg}
% }
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{application-figures/cockpit-10-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/cockpit-3-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/cockpit-4-1.jpg}
% }
% \caption{}
% ~\label{fig:application-cockpit}
% \end{figure}


% \begin{figure}[h!]
% \centering
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{application-figures/body-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/body-2.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/body-3.jpg}
% }
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{application-figures/body-1-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/body-2-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/body-3-1.jpg}
% }
% \caption{}
% ~\label{fig:application-body}
% \end{figure}

% \subsection{Basic UI Elements}

% \subsubsection{Buttons, Sliders, and Knob}

% \begin{figure}[h!]
% \centering
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{application-figures/mountain-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/mountain-3.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/mountain-4.jpg}
% }
% \resizebox{1\columnwidth}{!}{
% \includegraphics[height=1\textwidth]{application-figures/mountain-1-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/mountain-3-1.jpg}
% \hspace{0.1cm}
% \includegraphics[height=1\textwidth]{application-figures/mountain-4-1.jpg}
% }
% \caption{}
% ~\label{fig:application-mountain}
% \end{figure}



%\begin{figure}[t!]
%\centering
%\resizebox{1\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{application-figures/house-7.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/house-6.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/house-4.jpg}
%}
%\resizebox{1\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{application-figures/house-7-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/house-6-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/house-4-1.jpg}
%}
% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.6\columnwidth]{draft-figures/App_House.jpg}
% \caption{Modeling a virtual environment: Users touch and rearrange 3D models by handling the robots.}
% ~\label{fig:application-house}
% \end{figure}



%Changed from: Games like Minecraft often rely on players constructing upon pretended physical entities. However they lack the haptics hinders their experience. The use of \system{} can greatly amplify construction mode or game play in existing VR games. A part from the previously mentioned scenarios of grab, push, and encounter, multiple robots can act in coordinated ways and simulate larger objects (Figure \ref{fig:application-minecraft}).

%\begin{figure}[h!]
%\centering
%\resizebox{1\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{application-figures/minecraft-3.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/minecraft-4.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/minecraft-2.jpg}
%}
%\resizebox{1\columnwidth}{!}{
%\includegraphics[height=1\textwidth]{application-figures/minecraft-3-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/minecraft-4-1.jpg}
%\hspace{0.1cm}
%\includegraphics[height=1\textwidth]{application-figures/m%inecraft-2-1.jpg}
%}





% Section-7 FUTURE WORK


% \subsubsection*{Multi-axis Tilt Support}
% Currently, \system{} can only tilt along one axis, requiring robots to move and rotate to render the other axis.
% One solution to avoid this problem is to use a multi-axis tilting mechanism like~\cite{alexander2012tilt}, but it introduces a challenge of miniaturization.
% Another potential solution of this is to use an omni-directional robot as a base part, instead of the current Toio robot.
% This might include Omni wheels~\footnote{\url{https://en.wikipedia.org/wiki/Omni_wheel}} or Mecanum wheels~\footnote{\url{https://en.wikipedia.org/wiki/Mecanum_wheel}} mechanisms.
% The multi-axis tilt support would enable the more expressive capability of \system{}, but we need more future work to address this problem.

% \subsubsection*{Different Form Factor}
% Our distributed encountered-type haptic concept is not bound to our specific implementation.
% For example, it would be interesting to explore different form factors of robots, such as the combination of robotic arms and mobile robots, instead of our height-changing robots.
% The comparison of these two different configurations would introduce an interesting trade-off, which relates to our design choice of using a swarm of simple robots, rather than few complex ones. 
% For example, mobile robotic arms could allow more degree of freedom thus expressive haptic experiences, but since it requires complex path planning in 3D space, rather than in 2D space, it would become more challenging to increase the number of such mobile robotic arms.
% On the other hand, a simple shape-changing robot can be limited with its expression capability, but by leveraging coordinated behaviors, these robots can generate various haptic sensations as demonstrated in the paper.
% Future work should further explore the broader design space of our proposed approach to better understand these advantages and trade-offs.



% \subsubsection*{Vertical Surface}
% While the robot can currently move only on a horizontal surface, we expect it is also possible to move on a vertical surface with appropriate infrastructure.
% Such robots can augment the various existing encountered-type haptic devices (e.g., Sparse Haptic Proxy~\cite{cheng2017sparse}).
% We have tested whether the robot can stick and move onto a vertical surface with a magnetic plate and attached with a strong magnet, but the initial simple experiment did not work well because we observed the stronger magnet makes it difficult for robots to move, while the weaker magnet is too weak to hold the robot from gravity.
% However, we anticipate the different form factors of robots or different locomotion systems (e.g., using strings or X-Y plotter) enable vertical locomotion. 
% Since our linear actuator is compact, modular, and lightweight, it is also possible to explore the vertical shape display.
% We are interested in how these augmentations can broaden the design space and application scenarios.



%\eyal{Eyal: What about limitations of continuous touch while the robots are moving: 
%a. There is no friction between the hand and the robot's top surface. We could address that in the future.
%b. The robots latency, acceleration \& deceleration might reduce believabillty.}

%\eyal{Eyal: A few more future work:
%a. Better anticipation of potential touch events, using the user's behaviour such as eye-gaze, or by context of the application.
%b. Additional strategies for swarm robot movement, such as covering possible extension of touch between robots, or generating concurrent haptic feedback over multiple fingers .}

% \subsubsection*{Inter-material Interaction}
% In the literature of shape-changing interfaces, inter-material interaction refers to an interaction between active actuated elements and passive static objects [???].  \Mike {reference?}
% This type of actuation has been greatly explored in the domain of shape-changing interfaces (e.g., inFORM, Sublimate) or actuated tangible interfaces (e.g., Molebots). 
% \system can leverage this inter-material interaction to expand the design space of haptic interactions. 
% For example, by actuating flexible fabric on top of the robot's top surface, these robots can create a continuous surface on which the user can touch and feel.
% Additional possibilities can realized by using the robots as actuators that move other static haptic objects around the interaction surface.
% %Also, these actuated surface can move a static passive ball and props, which can expand the interactions.



% For example, to enable multiple concurrent touch points, it would require multiple robot arms approaching the same space without intersecting or limiting the user’s hand motion, which is technically complex to achieve. In contrast, the HapticBots control and fabrication is fairly simple.

% For example, it would be interesting to know how we can free the limitation of mid-air haptics with a swarm of drones or robots that are attached to the ceiling.
% The use of drones for haptics have been explored recently~\cite{abtahi2019beyond, hoppe2018vrhapticdrones}.
% By building on top of these emerging haptics approaches, we can further explore this domain.
% As future work, we are interested in further exploring different form factors of robots to expand the range of applications.

% \subsubsection*{Graspable Shape-changing Haptics}
% One of the unique features of \system{} is its graspability.
% In the literature, current haptic devices are classified as either handheld devices or encountered-type devices.
% In future work, we are interested in how we can integrate the collective mobile robots to transform into shape-changing handheld haptic devices.
% For example, similar to the Robotic Assembly~\cite{zhao2017robotic}, we envision multiple \system{} robots to assemble and connect to become a handheld object.
% The current implementation does not fully support rich interactions while grasping, we will further explore to integrate these two domains with one unified platform.



%Possibly using different coverings on the top of the robots could further increase the haptic experience with more compatible textures. 
%We envision using coverings for the mechanisms or multiple bots that would allow participants to grab the HapticBots safely. As well as render more complex or larger objects.
%}


% Toio robot cannot move in an arbitrary direction, as the drivetrain is based on two parallel wheels.
% This limits how the robot can tilt its top surface in an arbitrary direction while moving to a target location. 
% Instead, it has to rotate in place to change the orientation of the top cap after it has reached the target location. 
% To avoid this issue, we are interested in exploring an omni-directional robot as a base part. 



%Mike  Tabletop surface? Higher resolution than what? Current shape display - HapticBots?
% On the other hand, we also noticed the small size robot requires more precise control of both position and height of the actuator, as it can easily produce the gap between two robots.
%\eyal{Eyal: I would not say this: All sizes need good control. 
%Large areas reduces the chances to touch a gap, but then there may be a limit in expressivity too}
% In contrast, the larger touch surface area makes it difficult to produce complex shapes, but it can support many fingers with the smooth touch surface.
% Therefore, it is an interesting discussion about what might be a practically good size for the VR haptics application.

% In addition, as the size of the robots decreases, the system may also need to support more robots, which requires more sophisticated swarm controls.


% Due to this limitation, we used the Oculus controller as an external handheld tool to interact with robots (e.g., a hammer in Minecraft, a sculpting tool for 3D modeling), but a


% this inter-material interaction to expand the design space of haptic interactions. 
% For example, by actuating flexible fabric on top of the robot's top surface, these robots can create a continuous surface on which the user can touch and feel.
% Additional possibilities can realized by using the robots as actuators that move other static haptic objects around the interaction surface
% In the literature of shape-changing interfaces, inter-material interaction refers to an interaction between active actuated elements and passive static objects [???].  \Mike {reference?}
% This type of actuation has been greatly explored in the domain of shape-changing interfaces (e.g., inFORM, Sublimate) or actuated tangible interfaces (e.g., Molebots). 
%Also, these actuated surface can move a static passive ball and props, which can expand the interactions.





%\eyal{Eyal: We must address this in the technical part: How fast can we go with entire mechanism? Did users found themselves limited for 'regular' motions? What if we choose a setup that somewhat limits the user speed such as siting on a chair in front of a desk with haptic display?}
%b. Additional strategies for swarm robot movement, such as covering possible extension of touch between robots, or generating concurrent haptic feedback over multiple fingers 

%Mike   Did you explore monitoring the motor cuttent in the actuators?


%  (Figure~\ref{fig:concept} bottom right). It may also open options such as adding physical widgets such as buttons.

